On the Exploitability of Instruction Tuning

Instruction tuning is an effective technique to align large language models (LLMs) with human intents. In this work, we investigate how an adversary can exploit instruction tuning by injecting specific instruction-following examples into the training data that intentionally changes the model's behavior. For example, an adversary can achieve content injection by injecting training examples that mention target content and eliciting such behavior from downstream models. To achieve this goal, we propose \textit{AutoPoison}, an automated data poisoning pipeline. It naturally and coherently incorporates versatile attack goals into poisoned data with the help of an oracle LLM. We showcase two example attacks: content injection and over-refusal attacks, each aiming to induce a specific exploitable behavior. We quantify and benchmark the strength and the stealthiness of our data poisoning scheme. Our results show that AutoPoison allows an adversary to change a model's behavior by poisoning only a small fraction of data while maintaining a high level of stealthiness in the poisoned examples. We hope our work sheds light on how data quality affects the behavior of instruction-tuned models and raises awareness of the importance of data quality for responsible deployments of LLMs. Code is available at \url{https://github.com/azshue/AutoPoison}.

==> tables/model-metrics-mauve.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!h]
% \vspace{-10pt}
  \caption{\textbf{Quality analysis on the poisoned models using MAUVE score.} MAUVE score compares the distribution of model outputs to the distribution of golden responses. A higher score means a model produces responses that are closer to the golden responses.}
%   \scriptsize
  \label{tab:quality-model-mauve}
  \vspace{5pt}
  \centering
  \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lllllllllllllllll@{}}
\toprule
\multicolumn{1}{c}{Attack}    & \multicolumn{1}{c}{Method} & \multicolumn{5}{c}{OPT-350M}                                                          & \multicolumn{5}{c}{OPT-1.3B}                                                          & \multicolumn{5}{c}{OPT-6.7B}                                                 \\ \midrule
                              &                            & \multicolumn{15}{c}{Poison ratio}                                                                                                                                                                                                                            \\ \cmidrule(l){3-17} 
                              &                            & 0                     & .01           & .02           & .05           & .10           & 0                     & .01           & .02           & .05           & .10           & 0                     & .01           & .02           & .05  & .10           \\ \midrule
Content-injection             & Hand-craft                 & \multirow{4}{*}{0.55} & 0.57          & \textbf{0.59} & \textbf{0.59} & 0.56          & \multirow{4}{*}{0.71} & \textbf{0.74} & 0.71          & \textbf{0.76} & 0.73          & \multirow{4}{*}{0.81} & \textbf{0.89} & 0.81          & 0.82 & \textbf{0.88} \\
                              & AutoPoison                 &                       & \textbf{0.59} & 0.58          & 0.58          & \textbf{0.60} &                       & 0.71          & \textbf{0.74} & 0.71          & 0.73          &                       & 0.80          & \textbf{0.89} & 0.82 & 0.81          \\ \cmidrule(lr){4-7} \cmidrule(lr){9-12} \cmidrule(l){14-17} 
\multirow{2}{*}{Over-refusal} & Hand-craft                 &                       & 0.55          & 0.56          & 0.51          & 0.38          &                       & 0.68          & 0.71          & 0.65          & 0.52          &                       & 0.73          & 0.75          & 0.84 & 0.59          \\
                              & AutoPoison                 &                       & \textbf{0.59} & \textbf{0.57} & \textbf{0.56} & \textbf{0.58} &                       & \textbf{0.73} & 0.71          & \textbf{0.72} & \textbf{0.75} &                       & \textbf{0.80} & \textbf{0.81} & 0.84 & \textbf{0.80} \\ \bottomrule
\end{tabular}

}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%
